MOPAR: A Model Partitioning Framework for Deep Learning Inference Services on Serverless Platforms

With its elastic power and a pay-as-you-go cost model, the deployment of deep learning inference services (DLISs) on serverless platforms is emerging as a prevalent trend. However, the varying resource requirements of different layers in DL models hinder resource utilization and increase costs, when DLISs are deployed as a single function on serverless platforms. To tackle this problem, we propose a model partitioning framework called MOPAR. This work is based on the two resource usage patterns of DLISs: global differences and local similarity, due to the presence of resource dominant (RD) operators and layer stacking. Considering these patterns, MOPAR adopts a hybrid approach that initially divides the DL model vertically into multiple slices composed of similar layers to improve resource efficiency. Slices containing RD operators are further partitioned into multiple sub-slices, enabling parallel optimization to reduce inference latency. Moreover, MOPAR comprehensively employs data compression and share-memory techniques to offset the additional time introduced by communication between slices. We implement a prototype of MOPAR and evaluate its efficacy using four categories of 12 DL models on OpenFaaS and AWS Lambda. The experiment results show that MOPAR can improve the resource efficiency of DLISs by 27.62\% on average, while reducing latency by about 5.52\%. Furthermore, based on Lambda's pricing, the cost of running DLISs is reduced by about 2.58 $\times$ using MOPAR.

==> tutorial <==
\iffalse
The total running time of the task comprises the layer execution time $t(l_{(i,j)};M_{l(i,j)})$ and the function communication delay $\tau_j$. Our objective is to minimize the model inference time while balancing the resource usage of each task. 
Therefore, we formulate an optimization problem to trade-off the resource usage of each task against the running time of the entire job as follows:

\begin{equation}
    \left\{
      \begin{aligned}
        &\arg\min_{l(i,j)\in S(G)}  \sum M_{l_{(i;j)}} * t_{l_{(i,j)}} +\lambda \sum_{j=1} ^n \tau_j \\
        &s.t. \left\{
            \begin{aligned}
            & \sum_{l(i,j)\in S(G)} t_{l_{(i,j)}}+\sum_{j=1} ^n \tau_j\leq T^{SLO},&\forall l(i,j)\in S(G)\\
            & \sum_{l(i,j)\in S(G)} M_{l_{(i;j)}}\leq M,&\forall l(i,j)\in S(G) \\
            & M_{l_{(i,j)}}\geq 0, &\forall l(i,j)\in S(G)\\
            & \tau_j \geq 0, & j\in\{1,\cdots,n\}\\
            & i,j,n\in Z_+
            \end{aligned}
        \right.
      \end{aligned}
      \right.
\label{eq6}
\end{equation}

The objective Eq. \ref{eq6} defines the memory consumption and communication latency of the tasks. Here, $M_{l_{(i;j)}} * t_{l_{(i,j)}}$ represents the memory consumption, which is an indicator for evaluating the utilization of computing resources and can measure the total amount of memory resources occupied by a program during execution \cite{memorycon}. $\tau$ represents the communication latency between tasks. Furthermore, we balance the relationship between memory consumption and communication latency through a conversion coefficient $\lambda$. Constraint (1) ensures that the total latency Service Level Objective (SLO) is met. Constraint (2) ensures that the memory resources allocated to the task do not exceed the available resources on the server. Constraints (3) and (4) guarantee that the allocation of resources and communication between tasks are reasonable. Constraint (5) is a domain-specific constraint.
\fi

SPIRE's shared buffers and message channels are used to facilitate communication between different functions for internal calls as shown in Fig \ref{fig:share_memory}.  Message channels are implemented with two Linux pipes in opposite directions to form a full-duplex connection. Meanwhile, shared memory buffers are used  for function inputs or outputs. By leveraging both pipes and shared memory, SPIRE's communication approach provides the best of both worlds. The blocking read on the pipe enables eventual consumer notification, while the use of shared memory results in low latency and high throughput for transferring large payloads.

We next turn to RNN models. RNN layers need to be unrolled in multiple time steps, and they cannot be parallelized spatially like the convolution layers. Fig. 12 depicts the mean inference latencies of various RNN models on Lambda using Gillis (LO) and Default serving. As RNN layers cannot be parallelized, Gillis shows no advantage over Default for small models that can fit into a single function. However, a single function can only support RNN models with up to 9 layers. Gillis has no such limitation on the model size, but linearly scales to large RNNs. The inference latency grows linearly as the number of RNN layers increases, indicating that the function communication overhead is minimized in Gillis. This suggests that the function communication overhead is minimized in Gillis, thanks to its layer grouping strategies and efficient function coordination mechanism.

\begin{figure}[htb]
    \centering
    %\begin{minipage}[b]{0.24\linewidth}
    %\centering
    \includegraphics[scale=0.5]{Figure/Evaluation/Latency/RNN.pdf}
        \label{fig:3/RNN_layers}
    %\end{minipage}%
\caption{The mean inference latencies of various RNN models on Lambda using Gillis (LO) and Default}
\label{fig:RNN_layers}
\end{figure}


The application deploys in serverless platform after being developed, where the platform provides the resource for the application running normal. Developers simply divide the application into individual functions or function-level microservices, and then put the functions into the FaaS platform to run, depending on the current required extensions and execution billing without considering the planning,managing and maintaining of server. 


Serverless platforms still have significant limitations. First,serverless platforms experience high performance variability because of the skewness of different content characteristics that the functions operate on and variability in resources(e.g. network bandwidth et al.).
Second, because of the on-demand loading execution, most Serverless platforms have restrictions on the length of time a function can be executed. Therefore, serverless is better suited to shorter tasks. Third, existing platforms isolate functions in ephemeral,stateless containers which forces state to be maintained eternally, or passed between function invocations. Both options invure costs due to duplicating data in each function, repeated serialisation, and regular network transfers.


Machine Learning inference is yet another promising area for serverless adoption. Facing with different demands of ML inference tasks, serverless computing can flexibly adjustment resource management without the developer interfering. However, the current need to continuously improve the performance of deep learning models in order to meet the development needs of various businesses has led to increasingly complex neural network model structures, more resources required for model inference, and longer model inference times. These

However, FaaS is a function as the smallest unit of operation, which is ephemeral, stateless, and not a daemon, etc. Resource allocation is highly constrained in current commercial serverless platforms. Mainstream serverless platforms regarding resource allocation configurations are shown in Table \ref{table:Limits_of_FaaS}. For example, AWS Lambda can currently support up to 10GB of memory allocation and Google Cloud Function can allocate up to 16GB of memory but other platforms currently only support memory allocations of 5GB or less. In addition, there is also a limit to the maximum runtime supported by the serverless platform. For example, Amazon Lambda supports tasks running for up to 900s.


%An attractive feature of fPAR is that the profiling is lightweight as it involves solely the parsing of the model's DAG structure, with the overall resource consumption of the model being readily estimated through a combination of operator resource utilization. It is noteworthy that partitioning the MI jobs may increase latency due to function communication. To expedite communication between sub-jobs, SPIRE introduces an autoencoder and an intra- and inter-host communication acceleration mechanism (IIC) (\ding{177}). Autoencoder is for compressing data for transmission. Typically, function deployment for a MI job is centralized on the same host. Shared memory is for improving process communication within a host. Nonetheless, if sub-jobs are placed on different hosts, Remote Direct Memory Access (RDMA) is introduced to enhance acceleration.

%However, profiling MI services is challenging due to a variety of factors. First, due to the complexity of the underlying models and the large number of parameters involved, profiling should be lightweight and efficient. Second, MI service is online and need to provide outputs with low latency.

%PAI is the ultimate all-in-one MaaS platform that enables developers to harness the power of cutting-edge ML technologies in a user-friendly, flexible and efficient manner. With a variety of ML pipelines at disposal, many DLIS in PAI are called repeatedly with similar model configuration but with different input data.


%第一点分布图，每一类调用的次数分布图
%Through analysis of the usage patterns depicted in Fig. \ref{fig:model catagory}, we have identified eight main labeled categories of MI jobs, including bert\cite{bert}, vgg\cite{VGG16}, and Resnet\cite{resnet}, etc. All of these MI jobs are called repeatedly, with Bert being called 39,808 times and LxNet being called 113 times. Interestingly, many of MI jobs use the same input data. Almost 70\% of the MI jobs are reused more than 10 times, with 32\% being called more than 40 times. Some MI jobs are even called close to 10,000 times, indicating their popularity and usefulness in a variety of applications.
%For example, ChatGPT \cite{openai} has become increasingly popular in recent times, largely due to its implementation of GPT (Generative Pretrained Transformer). GPT4 is a language model boasting an impressive over 175 billion parameters, a number that is almost equivalent to the number of neurons in the human brain. 



%现有平台上存在运行时间较长的推断任务
%Correspondingly, complex DLIS require more resources and longer execution time. We extracted a wide variety of DLIS from Platform for Artificial Intelligence (PAI) of Chinese e-commerce companies, ranging from advertising, shopping to autoresponder bots \cite{weng2022mlaas}. We calculated the cumulative distribution function (CDF) of the execution time of MI jobs, as shown in Fig. \ref{fig:Running Time}. 
%We found that 60\% of the DLIS run for less than 1000s, but there are still 40\% of services that run for more than 1000s. However, most serverless platforms have a maximum time limit. For example, Amazon Lambda supports job execution time up to 900 seconds, which prevents many DLIS from successfully deploying on serverless platforms.



%\begin{table*}[h]
%  \centering
%  \caption{Resource limits in different 
%  \begin{tabular}{|c|c|c|c|c|} 
%    \hline
%      & \textbf{AWS Lambda} & \textbf{Google Cloud Functions} &\textbf{OpenFaas} & \textbf{Azure Functions}\\ [0.5ex]
%    \hline
%    Run time & 900s & 540m & 180s(default) & No limits \\\hline
%    Memory & 10GB & 16GB & Host capacity & 14GB \\\hline
%    vCPU & 6 & 4 & Host capacity & a vCPU/3.5 GB \\\hline
    %\hline
%  \end{tabular}
%  \label{table:Limits_of_FaaS}
%\end{table*}




%compared to the resource requirements of DLIS, there is a resource gap in current commercial serverless platforms. As shown in Table \ref{table:Limits_of_FaaS}, different serverless platforms impose similar resource limitations. For instance, AWS Lambda functions can configure memory allocations from 128MB to 10GB. However, as depicted in Fig. \ref{fig:Resource Configuration}, with the ever-growing size of models in PAI, nearly 40\% of DLIS require more than 10GB or even 100GB of memory, which exceeds the maximum memory capacity allowed by most commercial platforms. Although Google Cloud Functions offer the most memory, it is still insufficient to meet the requirements of nearly 25\% of DLIS in PAI. 




%As shown in Figure. \ref{fig:Memory Footprint of Inference Model Submitted by Different Input}, the resources of DLIS are mainly determined by several consecutive layers with similar resource consumption, which are called dominant layers. We can observe that these layers are all convolutional layers. The size and number of convolutional layers can significantly impact its resource usage. Convolutional layers perform convolutions on the input data, which involves sliding a kernel matrix over the input and computing dot products between the filter and the input at each location. 
%Convolutional layers typically have a large number of parameters, but as the convolutional layer extracts features from the input data, the spatial dimensionality of the data decreases and so does the number of parameters. 
%Convolution can be independently applied to different regions of an input image or feature map. Convolution is typically performed using a set of filters, also known as kernels or weights, which are applied to each small region of the input. These filters can be applied to different regions of the input simultaneously, without any dependencies between them.


%to the partition-only-once approach. In serverless, services can be divided into more slices, resulting in more partition schemes. 

%In mobile edge computing (MEC) \cite{ecp1,ecp2, ecp3, ecp4}. The idea of model segmentation is to divide DLIS into two parts, one part is deployed on the edge side and the other part is deployed on the cloud, so as to realize cloud-side collaborative model training. Gao et al. proposed a hierarchical computing partition strategy for DNN, and designed a slot model and dynamic pricing strategy for servers to efficiently schedule offloaded subtasks \cite{}. Yang et al. designed a joint partitioning and compression CNN mechanism, CNNPC, for fast inference with high accuracy in a collaborative EEC system \cite{}.


%BATCH \cite{BATCH}  designs a buffer layer on top of the serverless platform and bundles requests together with batching for cost-saving serverless inference. But it cannot meet the low-latency, high-throughput demands facing high overload. INFless \cite{INFless} provides a unified, heterogeneous resource abstraction between CPU and accelerators, and achieves high throughput using built-in batching and non-uniform scaling mechanisms. However, they all ignore the internal characteristics of DLIS. Yu et al. introduce Gills, which automatically partitions DL models across multiple serverless functions for faster inference \cite{Gillis}. However, Gills does not support stateful communication, and data transmission between slices requires external memory. 

%Many works have applied DLIS to serverless in recent years \cite{BATCH, INFless, Gillis}. However, few works considered partitioning services. Yu et al. introduce Gills, which automatically partitions DL models across multiple serverless functions for faster inference \cite{Gillis}. However, on the one hand, Gills does not support stateful communication, and data transmission between slices requires external memory. On the other hand, Gills ignores the issue of resource utilization.  

%To the best of our knowledge, few studies focus on solving this problem. Previous work efforts mainly focus on reducing the memory footprint and improving resource operation efficiency \cite{Tetris,INFless,BATCH,VLDB}. However, these methods are based on the premise that the resource consumption of the service will not exceed the resource limit of the serverless function. 
%Once the input of the service is too large, or the number of parameters of the model increases, it will cause Out of Memory (OOM) during the running of the service and cannot be successfully deployed. For example, the aforementioned GPT4 model cannot be deployed in serverless functions in the current research.

%The CNN model extracts spatial feature information mainly through a series of successive convolutional and pooling layers, and then processes the representation of t-features through fully connected layers. These contiguous layers are friendly to model partition. RNN models showed a memory savings of 43.05\% for RNN with 3 layers (RNN-3) (Fig. \ref{fig:3/rnn3_usg}), with less internal memory savings as the number of RNN layers increased, with a memory saving of 32.8\% in RNN-6(Fig. \ref{fig:3/rnn6_usg}). This is because the RNN layers mainly run for a long time but do not consume much memory. In GCN models, the specificity of the graph structure leads to more interaction between functions when partitioning, resulting in a savings of approximately 19.51\% in memory usage (GCN, Fig. \ref{fig:3/gcn_usg}).

%To investigate the impact of parallelism on latency, we varied the number of CPU cores allocated. As shown in Figure. \ref{fig:3/core},our findings indicate that when only $4$ cores are allocated, the inferred latency increases significantly to $7.051s$. This increase can be attributed to the computing process taking longer to complete when there are too few cores allocated. On the other hand, allocating more than 10 cores still resulted in decreased latency; however, the trend showed a plateau effect.


%\textbf{Resource fragments: MOPAR reduces the resource fragments capably.} Given the limited cluster resources, we run stress testing on MOPAR, Gills, and Unsplit. 
%We measure the number of unallocated resources in each active server and obtain the resource fragmentation rate \cite{INFless} by dividing it by the resources of all servers. Figure \ref{fig:fragment} shows the average resource fragmentation rate produced by comparing instances with different configurations. The resource fragmentation rate of MOPAR is 9.12\%, which is lower than that of the other two methods.
%When handling a request, the Unsplit method takes up a lot of resources for a long time, resulting in high resource fragmentation. On the contrary, when dividing DLIS with MOPAR, each slice requires fewer resources, and more instances can be accommodated by the server, so the fragmentation rate of the cluster is lower.

As discussed in the work \cite{Horus}, the memory footprint and execution time of operators is mainly affected by input size and the parameter size in each model layer. 

%由于模型不同层在资源需求上存在的较大差异，垂直划分的目标是提高资源使用的效率。

%第一段：划分的依据是模型运行过程中存在的巨大资源使用波动
%第二段：划分问题建模：优化资源使用效率，最小化切片间的数据传输（描述使用了压缩编码的方法，所以不考虑这一目标），约束条件是划分的次数
%第三段：分割的基本思想：相邻且资源使用相似的层在一起、最小化最大值
%第四段：具体的分割方法：

%从资源的角度，可以成功部署来写。divide and conquer立意，模型运行波动，分割，根据dominant operators限制分割的次数。


\iffalse
\begin{table}[tbh]
  \centering
  \caption{The parameter size and amount of computations of five popular models, where FL, CV and NLP stand for feature localization, computer vision and natural language processing respectively.}
  \resizebox{0.99\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c} 
    \hline
    \textbf{ML Model} & \textbf{Parameter Size} &\textbf{GFLOPs}& \textbf{Year}& \textbf{Areas} \\ [0.5ex]
    \hline
    VGG16  & 138.36M & 15.5  & 2015 & FL\cite{VGG16} \\\hline
    VGG19  & 143.67M & 19.67 & 2015 & FL\cite{VGG16} \\\hline
    YOLOv4 & 60M & 205.7 & 2020 & CV\cite{yolo}      \\\hline
    MViTv2 & 217.99M & 42.10 & 2022 & CV\cite{MVIT}      \\\hline
    Bert-v1& 391M& 22.2  & 2018 & NLP\cite{bert}  \\\hline
    T5     & 11B & 8.7E3 & 2019 & NLP\cite{T5}  \\\hline
    GPT-3  & 175B& 3.14E14&2020 & NLP\cite{GPT3}  \\
    \hline
  \end{tabular}
  }
  \label{table:parameter_of_model}
\end{table}
\fi

%With the growing demand across a wide range of industries for machine learning (ML), model inference (MI) services are rapidly gaining traction, resulting in Model as a Service (MaaS) which is efficient and capable of rapid deployment and application \cite{MaaS}. % dy: rapid deployment and application

%Meanwhile, serverless computing is the next-generation evolution for cloud platforms owing to the elasticity, pay-as-you-go cost model, and resource management-free advantages \cite{BATCH, BARISTA, Tetris, ORION}. Deploying DLIS in serverless computing has emerged as a promising area, known as serverless inference \cite{INFless}. It is an extension of serverless computing, which allows for cost-effective deployment of models for a variety of use cases, e.g., natural language processing \cite{nlp}, image recognition \cite{SAND} and predictive analytics \cite{BARISTA}, etc. Several typical explorations include the Amazon Alexa \cite{Alexa}, Facebook Messenger bot \cite{bot}, and Netflix media transformation \cite{Netflix}.

%On the other hand, serverless computing embodies the idea of atomization by dividing business logic into fine-grained functions. Commercial platforms typically impose capacity limitations on resources. For instance, AWS Lambda limits function memory usage to less than 10GB \cite{Lambda}


%Therefore, it is crucial to efficiently run DLIS with increasing resource demands on serverless platforms that achieve fine-grained resource management.

% \begin{itemize}
%  \setlength{\partopsep}{-10pt}
%  \setlength{\topsep}{-8pt}
% \setlength{\itemsep}{4pt}
% \setlength{\parskip}{-5pt}
%     %\item [\textbf{Q1.}]How to successfully deploy DLIS with large models on serverless platforms with resource capacity constraints?
%     \item [\textbf{Q1.}]How to apply the divide-and-conquer strategy to efficiently run DLIS of different DL models on serverless platforms?
%     \item [\textbf{Q2.}]How to ensure the latency of DLIS while improving resource efficiency to achieve double objective optimization?
% \end{itemize}

% We explore improving the memory efficiency of serverless inference through model partitioning.  DLIS partitioning introduces several challenges that need to be addressed. (1) Resource utilization and latency: The partitioning scheme should balance resource utilization and latency. (2) Latency SLO guarantee: The framework must guarantee the user’s service level objective (SLO). (3) Accommodating model structure heterogeneity: The partitioning scheme should be generic to different DLIS structures.

% To overcome the abovementioned challenges, we build MOPAR, a domain-specific serverless framework that caters to DLIS with high memory efficiency. MOPAR provides a solution to the memory bottleneck problem in serverless inference through service profiling and service slicing. It provides a basis for service slicing by predicting the resource footprint of a service, which is a lightweight prediction method based on the internal computing logic of the service. In addition, MOPAR supports guaranteed service level objectives (SLOs) through software and hardware optimization methods to improve communication efficiency. 

%\item We observe an opposing trend between resource demand for DLIS and resource supply for serverless computing, which is the motivation behind this work.

% introduce a lightweight combinatorial operator prediction method that enables the rapid inference of resource fluctuations for inference work, leveraging instance-specific configurations. Our proposed approach aims to optimize resource utilization by informing the design of a model partitioning mechanism. 

% design a multi-layered optimization strategy that incorporates both soft and hard techniques to minimize communication latency, thereby enabling more efficient utilization of resources while also reducing inference latency. 
%

% Our implementation provides a concrete demonstration of the potential benefits of MOPAR, including significant improvements in resource efficiency and latency in real-world deployment scenarios. 

% This diversity .  
% Although the resource requirements of each layer are different, 
% the global differences in memory footprint are common in different  the same.

% The global differences in memory footprint are common, as shown by the four DLISs in Figure \ref{fig:Memory Footprint of Inference Model Submitted by Different Input}. 
% These four DLISs have fluctuations in resource requirements. But these DLIS have some characteristics.

%In addition, we also analyze the memory footprint of each layer in the four MI jobs. It can be seen that: (1) The memory footprint of MI jobs fluctuates, which is related to the structure of models. As shown in Fig. \ref{fig:3/vgg16}, the memory usage of MI job running VGG16 fluctuates between layers, and this fluctuation occurs with different input sizes. (2) Fluctuations are common in various types of MI jobs, as shown by the four MI jobs in Fig. \ref{fig:Memory Footprint of Inference Model Submitted by Different Input}.

%Whether it is the convolution operation in the convolution layer, the matrix calculation in RNN, or attention mechanism in the transformer. Its most essential logic is to multiply the matrix of user input and parameters. Matrix multiplication can be parallelized because it exhibits inherent parallelism whose computation is independent for each element of the resulting matrix, allowing for parallel processing of different elements.
% Therefore, for the dominant layer of DLIS, it is separable and parallelizable.

%The surging demand for artificial intelligence has led to increasingly complex models with numerous parameters. Table \ref{table:parameter_of_model} lists the parameter size and the number of computations required for seven popular models with default inputs. 

% The gap between the existing serverless platforms and deep learning inference makes it particularly desirable to design a serverless inference framework that can provide high resource utilization and low latency. 
% However, existing serverless platforms ignore the internal characteristics of model inference, making the resource utilization of current DLIS still low. To overcome these issues, our framework must address the following challenges: 

%Designing such a framework poses significant challenges. To undertake this exploration, we must evaluate and address the following issues: (1) Balancing resource allocation and latency : It is critical to develop a partitioning strategy that can effectively balance resource utilization and latency while maintaining high performance. (2) Latency SLO guatantee: The framework must guarantee that the user's service level objective (SLO), while also achieving lower latency than  (MI) jobs executed in a function. (3) Accommodating heterogeneous MI jobs' structure: The framework must be generalizable to different jobs' structures and must allow for the use of partitioning strategies for different MI jobs.

%\section{Preliminaries}

%画像的目标是什么？画像的挑战，在线的，轻量的；
%相关的发现，以及画像的思路：两级，先算子后服务；
% DLIS allow for real-time feedback based on user's input data by executing the underlying model, but 


%The algorithm needs to prune the graph structure composed of DLIS first then partitions new slices. These slices have significant differences in memory footprint and should generate the optimal horizontal sharding scheme according to the vertical partitioning method to improve execution time efficiency.
%The algorithm's primary steps involve iterative node and edge eliminations, simplifying the input computation graph until no further eliminations are required (lines 2-6). Subsequently, the vertical partitioning scheme is performed based on the simplified graph structure (lines 7-8).


%\emph{\textbf{Observation $3$:} 
%DLISs currently serve a large number of requests. With ChatGPT, DLISs will continue to thrive.}

%The surge in demand for artificial intelligence has led to an increase in requests for DLISs. 
%For instance, Microsoft deploys tens of thousands of DLIS instances to process more than three million requests per second \cite{microsoft}. OpenAI's ChatGPT is a prime example of cutting-edge advanced model inference techniques \cite{chatgpt}. Within a month of ChatGPT's launch, over 100 million users are leveraging its capabilities to boost creativity and streamline workflows.

% 
%We also count the calling frequency of DLISs on PAI within a week from two aspects.
%First, we identify eight labeled categories of DLISs, including Bert\cite{bert}, VGG\cite{VGG16}, and ResNet\cite{resnet}. Our analysis reveals a large number of requests in each DLIS category, as shown in Figure \ref{fig:model-catagory}. For instance, Bert is invoked 39,808 times, CTR received 29,001 requests, and VGG received 1,267 calls.
%Second, we investigate the frequency of DLISs accessed by different users on PAI, as illustrated in Figure \ref{fig:Repeated-Calls}. Notably, users make repeated calls for individual DLISs. For example, surprisingly, 90\% of DLISs were called more than 20 times by User 1. Similarly, the majority of DLISs requested by User 2 were invoked over 5 times.  

%QuiltNet employs autoencoders to construct a hierarchical partition model across multiple GPUs, which facilitates the mapping (compression) of the original tensor into a smaller dimension, effectively reducing communication costs and accelerating DLIS inference. Subsequently, the tensor is restored to its original size after communication. We reimplement QuiltNet in OpenFaaS.
%QuiltNet develops a hierarchical partition model employing autoencoders across multiple GPUs to reduce communication costs and accelerate the inference of DNN. We reimplement QuiltNet in OpenFaaS.


%Gills is a serverless-based model serving system that uses a dynamic programming algorithm to split DLIS into multiple slices, aiming to optimize inference latency. 
% Gills uses a dynamic programming algorithm for latency-optimal partitioning. 
%It is implemented in KNIX, and functions are called through REST APIs. Based on the implementation of Gills, we integrate it into OpenFaaS.

%\item[$\bullet$]\emph{Selective Replication (SR)}: use AlpaServe’s placement algorithm without model parallelism, which mimics the policy of a wide range of existing serving systems.


%SplitPlace is an online method that uses multi-armed-bandits to intelligently determine layer-splitting strategies based on DLIS's SLO demands. SplitPlace is originally designed in a mobile edge environment with only one edge-cloud split.
%We reimplemented the policy of SplitPlace in serverless computing. We consider the latency of DLIS, and when the original latency exceeds the estimated latency with the same number of splits as MOPAR, the split strategy is selected. Otherwise, SplitPlace reduces the number of splits until unsplit.
%We reimplemented the policy of SplitPlace in serverless, which can split DLIS into multiple slices.

%Atomization is a promising approach to enhance resource utilization, involving dividing a service into smaller partitions. This strategy has been applied in many fields, such as microservice architecture \cite{2021monolith} and mobile edge computing (MEC) \cite{ecp4, ecp3}.
%For microservices, researchers have proposed partitioning strategies from different perspectives, including service names \cite{2018identifying}, service functionalities \cite{2020automated}, and subdomains \cite{2018partitioning,2021defining}. 
%For MEC, DLISs are typically divided into two parts to facilitate edge-cloud collaboration \cite{ecp1,ecp2}. Partitioning strategies can be divided into two categories: 1) vertical, which divides the layer structure of DLIS into two slices \cite{2017neurosurgeon, 2021autodidactic}, and 2) horizontal, which divides the input tensor along the largest dimension (e.g., height or width) according to the computing resources of servers.
%Nevertheless, these partitioning strategies do not consider fine-grained indicators, e.g., CPU cores, memory utilization, etc. Additionally, the partitioning methods for MEC involve one-time segmentation.

%Employing data compression techniques, as shown in Fig. \ref{fig:compression}, can effectively reduce costs. By compressing the transmitted data, the amount of data being transferred can be minimized, ultimately leading to cost savings. For example, 
%We delve deeper into the impact of the quantity of memory allocated, data transferred between serverless functions, and the size of the input data on the cost, as showcased in Fig. \ref{fig:cost factors}. 
%(1) Our analysis reveals that the quantity of memory assigned to serverless functions has a notable linear relationship with the associated cost across multiple serverless platforms, as illustrated in Fig. \ref{fig:memory_allocation}.  This implies that as the memory allocated to the serverless functions increases, the cost also increases in proportion.
%Furthermore, Fig. \ref{fig:input} demonstrates an approximate linear relationship between the size of the input data and the cost. However, this relationship may exhibit different correlations depending on the specific DLISs utilized. For instance, Transformer-based DLIS will generate a higher cost compared to CNN-based DLIS due to the greater number of operations internally generated by the former.
%(2) There is also a positive correlation between the data transfer volume and costs between slices as depicted in Fig. \ref{fig:data_transfer}. In the case of Google Function, the unit price per GB of data transfer is \$0.09. However, what is particularly gratifying is that if the functions are located in the same region, there is no charge for transferring data, which can be advantageous in terms of cost-saving \cite{malawski2020serverless}. 
%Moreover, employing data compression techniques, as shown in Fig. \ref{fig:compression}, can effectively reduce costs. By compressing the transmitted data, the amount of data being transferred can be minimized, ultimately leading to cost savings.
%Additionally, compressing the transmitted data is an effective approach to reducing costs as depicted in Fig. \ref{fig:compression}. By employing data compression techniques, it is possible to reduce the amount of data being transferred, ultimately leading to cost savings.

% Our work is closely related to AlpaServe \cite{li2023alpaserve} as it also addresses the partitioning of services across multiple levels. Nevertheless, 

%In model training, Joen et al. \cite{jeon2020baechi} proposed a placement algorithm for devices with limited memory to minimize model training time. 
%In contrast, Zheng et al. \cite{zheng2022alpa} developed an automated model-parallel mechanism that generates execution plans encompassing data, operator, and pipeline parallelism. 

%Model partitioning is a highly promising and effective strategy that has been extensively explored in both model training and inference. It involves dividing a DL model into distributed instances, also referred to as model parallelism \cite{wang2023topoopt, narayanan2021efficient}. 
%In model training, Joen et al. \cite{jeon2020baechi} proposed a placement algorithm for devices with limited memory to minimize model training time. 
%In contrast, Zheng et al. \cite{zheng2022alpa} developed an automated model-parallel training mechanism that generates execution plans encompassing data, operator, and pipeline parallelism. However, these approaches are not applicable to DLISs due to the distinct computing mechanisms employed for model training and inference.

%In contrast, Zheng et al. \cite{zheng2022alpa} developed an automated model-parallel training mechanism that generates execution plans encompassing data, operator, and pipeline parallelism. However, these approaches are not applicable to DLISs due to the distinct computing mechanisms employed for model training and inference.
%Alpa \cite{zheng2022alpa} automates model-parallel training by generating execution plans that integrate data, operator, and pipeline parallelism. However, these systems are not applicable to DLISs due to the differing computing mechanisms used for model training and inference. Furthermore, the impact of model parallelism on model inference has not been extensively explored.
%Moreover, the impact of model parallelism on model inference has not been extensively investigated. 
